Fourier approximation of the statistical properties of Anosov maps on tori

We study the stability of statistical properties of Anosov maps on tori by examining the stability of the spectrum of an analytically twisted Perron-Frobenius operator on the anisotropic Banach spaces of Gou\"ezel and Liverani. By extending our previous work in [8], we obtain the stability of various statistical properties (the variance of a CLT and the rate function of an LDP) of Anosov maps to general perturbations, including new classes of numerical approximations. In particular, we obtain new results on the stability of the rate function under deterministic perturbations. As a key application, we focus on perturbations arising from numerical schemes and develop two new Fourier-analytic method for efficiently computing approximations of the aforementioned statistical properties. This includes the first example of a rigorous scheme for approximating the peripheral spectral data of the Perron-Frobenius operator of an Anosov map without mollification. Using the two schemes we obtain the first rigorous estimates of the variance and rate function for Anosov maps.

==> naive_ng_ldp.tex <==
\section{Large Deviations under the naive Nagaev-Guivarc'h method}\label{sec:ldp_naive_ng}

In this appendix we prove Theorem \ref{thm:naive_ng_ldp}; we assume the setting of the Theorem throughout.
Define $\Lambda: \R \to \R$ by
\begin{equation*}
  \Lambda(t) = \lim_{n \to \infty} \frac{1}{n} \ln\left(\E \left(e^{t S_n}\right)\right),
\end{equation*}
where $S_n$ is the partial sum of the sequence $\{Y_k\}_{k \in \N}$ from the statement of Theorem \ref{thm:naive_ng_ldp}.
The proof follows a well-trodden route (see e.g. \cite{hennion2001limit,Aimino2015}); we show that $\Lambda$ satisfies the requirements of the local Gartner-Ellis theorem Theorem \ref{thm:local_gartner_ellis} on some open real neighbourhood of 0.

\begin{theorem}[{\cite[Lemma XIII.2]{hennion2001limit}}]\label{thm:local_gartner_ellis}
  For all $n \ge 1$, denote by $\Prob_n$ a probability measure on some measurable space $(\Omega, \A)$, by $\E_n$ the corresponding expectation operator and by $S_n$ a real-valued random variable. Assume that for $t \in (-\theta, \theta)$, $\theta > 0$, we have
  \begin{equation*}
    \lim_{n \to \infty} \frac{1}{n} \ln\left(\E_n\left(e^{t S_n}\right)\right) = \Lambda(t),
  \end{equation*}
  where $\Lambda$ is strictly convex and $\mathcal{C}^1$ on $(-\theta, \theta)$, $\Lambda'(0) = 0$. Let $r : (\Lambda'(-\theta), \Lambda'(\theta)) \to \R$ be the convex conjugate of $\Lambda$ i.e.
  \begin{equation*}
    r(\epsilon) = \sup_{\abs{t} < \theta } \, (t \epsilon - \Lambda(t)).
  \end{equation*}
  Then $r$ is a non-negative, convex and continuous function that vanishes at 0, and, for all $\epsilon \in (0, \Lambda'(\theta))$, we have
  \begin{equation*}
    \lim_{n \to \infty} \frac{1}{n} \ln(\Prob_n(S_n > n \epsilon)) = -r(\epsilon).
  \end{equation*}
\end{theorem}

\begin{remark}
  Maybe some comments on the difference between the above statement and the version in Hennion/herve.
\end{remark}

\begin{lemma}\label{lemma:Lambda_spectral_formula}
  There exists $\theta > 0$ such that $\Lambda$ is finite and $\mathcal{C}^1$ on $(-\theta, \theta)$.
  \begin{proof}
    By \cite[Proposition 2.3]{gouezel2015limit}, there exists $\theta > 0$ and $\mathcal{C}^1$ maps $\lambda(\cdot): (-\theta, \theta) \to \C$, $\Pi(\cdot): (-\theta, \theta) \to L(E)$, and $N(\cdot): (-\theta, \theta) \to L(E)$, such that $(-\theta, \theta) \subseteq I$ and $A(t)$ is a simple quasi-compact with leading eigenvalue $\lambda(t)$ and decomposition $A(t) = \lambda(t) \Pi(t) + N(t)$ for every $t \in (-\theta, \theta)$.
    We will prove that
    \begin{equation}\label{eq:ldp_naive_ng_1}
      \Lambda(t) = \lim_{n \to \infty} \frac{1}{n} \ln\left(\E(e^{t S_n})\right) = \ln\abs{\lambda(t)}
    \end{equation}
    for every $t \in (-\theta, \theta)$, from which the required properties of $\Lambda$ follow straightforwardly.
    Fix $t \in (-\theta, \theta)$. Recall from the hypotheses of Theorem \ref{thm:naive_ng_ldp} that
    \begin{equation}\label{eq:mgf_quasicompact}
      \E(e^{t S_n}) = \nu A(t)^n \zeta = \lambda(t)^n \nu \Pi(t)\zeta  + \nu N^n(t) \zeta
    \end{equation}
    for every $n \in \N$.

    Since $\rho(N(0)) < \rho(L(0)) = 1$, we have $ \lim_{n \to \infty} \nu N^n(0) \zeta = 0$. Evaluating \eqref{eq:mgf_quasicompact} at $t = 0$ and letting $n \to \infty$, we find that
    \begin{equation*}
      1 = \lim_{n \to \infty} \lambda(0)^n \nu \Pi(0)\zeta.
    \end{equation*}
    Hence $\lambda(0) = 1$ and $\nu \Pi(0)\zeta = 1$.
    As $t \mapsto \lambda(t)$ and $t \mapsto \Pi(t)$ are $\mathcal{C}^1$ on $(-\theta, \theta)$, we may therefore shrink $\theta$ so that $\abs{ \nu \Pi(t)\zeta} > 0$ and $\abs{ \lambda(t)} > 0$ for every $t \in (-\theta, \theta)$.

    As $S_n$ is real valued, $\E(e^{t S_n}) > 0$. Thus $\ln(\E(e^{t S_n}))$ is well-defined and
    \begin{equation}\begin{split}\label{eq:ldp_naive_ng_2}
      \lim_{n \to \infty} \frac{1}{n} \ln\left(\E(e^{t S_n})\right) &= \lim_{n \to \infty} \frac{1}{n} \ln\left(\lambda(t)^n \nu \Pi(t)\zeta  + \nu N^n(t) \zeta\right)\\
      &= \Log\left(\lambda(t)\right) + \lim_{n \to \infty} \frac{1}{n} \Log\left( \nu \Pi(t)\zeta  + \frac{\nu N^n(t) \zeta}{\lambda(t)^n} \right) + \frac{2\pi i k_n}{n},
    \end{split}\end{equation}
    where $\Log$ is the principal value of the complex logarithm and each $k_n \in \Z$.
    By taking the real part of \eqref{eq:ldp_naive_ng_2} we obtain
    \begin{equation}\label{eq:ldp_naive_ng_3}
      \lim_{n \to \infty} \frac{1}{n} \ln\left(\E(e^{t S_n})\right) =  \ln\abs{\lambda(t)} + \lim_{n \to \infty} \frac{1}{n} \ln\abs{ \nu \Pi(t)\zeta  + \frac{\nu N^n(t) \zeta}{\lambda(t)^n} }.
    \end{equation}
    As $\rho(N(t)) < \rho(A(t)) = \abs{\lambda(t)}$, by the spectral radius formula it follows that $\lim_{n \to \infty} \frac{\nu N^n(t) \zeta}{\lambda(t)^n} = 0$. Recalling that $\abs{\nu \Pi(t)\zeta} > 0$, we therefore have
    \begin{equation*}
    \lim_{n \to \infty} \frac{1}{n} \ln\abs{ \nu \Pi(t)\zeta  + \frac{\nu N^n(t) \zeta}{\lambda(t)^n} } = 0.
    \end{equation*}
    Thus we obtain \eqref{eq:ldp_naive_ng_1} from \eqref{eq:ldp_naive_ng_3}, as claimed.
    As $t \mapsto \lambda(t)$ is $\mathcal{C}^1$ and $\abs{\lambda(t)} > 0$ for every $t \in (-\theta, \theta)$ it follows that $\Lambda$ is $\mathcal{C}^1$ on $(-\theta, \theta)$. That $\Lambda$ is finite on $(-\theta, \theta)$ is now clear.
  \end{proof}
\end{lemma}

\begin{lemma}\label{lemma:Lambda_deriv_at_zero}
  $\Lambda'(0) = 0$.
  \begin{proof}
    Recall from the proof of Lemma \ref{lemma:Lambda_spectral_formula} that for $t \in (-\theta, \theta)$ we have $\Lambda(t) = \ln \abs{\lambda(t)}$, where $\lambda(t)$ is an isolated simple leading eigenvalue of $A(t)$. Differentiating yields
    \begin{equation*}
      \Lambda'(t) =  \frac{ \frac{\mathrm{d}}{\mathrm{d}t} \abs{\lambda(t)} }{\abs{\lambda(t)}}.
    \end{equation*}
    Recalling from the proof of Lemma \ref{lemma:Lambda_spectral_formula} that $\abs{\lambda(0)} = 1$ and using the chain rule to evaluate $\frac{\mathrm{d}}{\mathrm{d}t} \abs{\lambda(t)}$ at $t = 0$,  we observe that is sufficient to prove that $\lambda'(0) = 0$.
    Recall that $\E(e^{tS_n}) = \nu A(t)^n\zeta$ for $t \in I$, and so the moment-generating function of each $S_n$ is finite in a neighbourhood of $0$. Hence, by standard properties of moment-generating functions,
    \begin{equation*}
      \E(S_n) = \lim_{t \to 0} \frac{\mathrm{d}}{\mathrm{d}t} \E(e^{tS_n}).
    \end{equation*}
    Now, for $t \in (-\theta, \theta)$ the operator $A(t)$ is quasi-compact with decomposition $A(t) = \lambda(t)^n \Pi(t) + N(t)$ where $\lambda(\cdot), \Pi(\cdot)$ and $N(\cdot)$ are all $\mathcal{C}^1$. Hence
    \begin{equation*}\begin{split}
      \frac{\mathrm{d}}{\mathrm{d}t} \E(e^{tS_n}) &= \frac{\mathrm{d}}{\mathrm{d}t} \left(\lambda(t)^n \nu\Pi(t)\zeta + \nu N(t)^n \zeta \right)\\
      &= n\lambda'(t)\lambda(t)^{n-1} \nu\Pi(t)\zeta + \lambda(t)^n \nu\Pi'(t)\zeta + \sum_{k= 0}^{n-1} \nu N(t)^{n-1-k} N'(t) N^k(t) \zeta .
    \end{split}\end{equation*}
    Recalling that $\lambda(0) = 1 = \nu\Pi(0)\zeta$ and letting $t \to 0$ we have
    \begin{equation}\label{eq:Lambda_deriv_at_zero_1}
      \E(S_n) = \lim_{t \to 0} \frac{\mathrm{d}}{\mathrm{d}t} \E(e^{tS_n}) = n\lambda'(0) +  \nu\Pi'(0)\zeta + \sum_{k= 0}^{n-1} \nu N(0)^{n-1-k} N'(0) N^k(0) \zeta.
    \end{equation}
    Let $r \in (\rho(N(0)), 1)$. By the spectral radius formula there exists some $C > 0$ such $\norm{N(0)^m} \le Cr^m$ for every $m \in \Z^+$. Hence there exists some $K > 0$ such that
    \begin{equation*}
      \abs{\sum_{k= 0}^{n-1} \nu N(0)^{n-1-k} N'(0) N^k(0) \zeta} \le  K n r^{n-1}
    \end{equation*}
    for all $n \in \Z^+$. In particular, by dividing \eqref{eq:Lambda_deriv_at_zero_1} by $n$ and then letting $n \to \infty$ we find that $\lambda'(0) = \lim_{n \to \infty} \E(S_n) / n = 0$, which concludes the proof.
  \end{proof}
\end{lemma}

\begin{proof}[Proof of Theorem {\ref{thm:naive_ng_ldp}}]
  Reviewing the proof of Lemma \ref{lemma:Lambda_spectral_formula}, we observe that $\Lambda(t) = \ln \abs{\lambda(t)}  = \ln \rho(A(t))$ for $t \in (-\theta, \theta)$.
  Thus, by the hypotheses of Theorem \ref{thm:naive_ng_ldp}, $\Lambda(t)$ is strictly convex in a neighbourhood $U$ of $0$.
  The restriction of $\Lambda$ to $(-\theta, \theta) \cap U$ satisfies the requirements of the local G\"{a}rtner-Ellis Theorem (Theorem \ref{thm:local_gartner_ellis}) by Lemmas \ref{lemma:Lambda_spectral_formula} and \ref{lemma:Lambda_deriv_at_zero}, and so $\{Y_k \}_{k \in \N}$ satisfies a large deviation principle.
\end{proof}

